Distance-generalized Core Decomposition

The $k$-core of a graph is defined as the maximal subgraph in which every vertex is connected to at least $k$ other vertices within that subgraph. In this work we introduce a distance-based generalization of the notion of $k$-core, which we refer to as the $(k,h)$-core, i.e., the maximal subgraph in which every vertex has at least $k$ other vertices at distance $\leq h$ within that subgraph. We study the properties of the $(k,h)$-core showing that it preserves many of the nice features of the classic core decomposition (e.g., its connection with the notion of distance-generalized chromatic number) and it preserves its usefulness to speed-up or approximate distance-generalized notions of dense structures, such as $h$-club. Computing the distance-generalized core decomposition over large networks is intrinsically complex. However, by exploiting clever upper and lower bounds we can partition the computation in a set of totally independent subcomputations, opening the door to top-down exploration and to multithreading, and thus achieving an efficient algorithm.

==> landmarks.tex <==
Landmarks-based indexes play an important role in point-to-point (approximate) shortest-path query~\cite{sommer2014shortest,Potamias:2009,akiba2013fast}.
The idea is as follows.
Given a graph $G = (V,E)$ a pair of vertices $s,t \in V$ and another vertex $u \in V$  which plays the role of \emph{landmark}, we can approximate the shortest path distance $d_G(s,t)$ from the distances $d_G(s,u)$ and $d_G(u,t)$ by means of the following inequalities:
$$
d_G(s,t) \leq d_G(s,u) + d_G(u,t)
$$
$$
d_G(s,t) \geq |d_G(s,u) - d_G(u,t)|
$$
Therefore, if we are given a set $L \subseteq V$ of $\ell = |L|$ landmarks we can bound the distance $d_G(s,t)$ as follows:
$$
\max_{u \in L} |d_G(s,u) - d_G(u,t)| \leq d_G(s,t) \leq \min_{u \in L} d_G(s,u) + d_G(u,t)
$$
In the following we use $L(s,t) = \max_{u \in L} |d_G(s,u) - d_G(u,t)|$ to denote the lower-bound and
$U(s,t) = \min_{u \in L} d_G(s,u) + d_G(u,t)$ to denote the upper-bound.

An interesting problem is how to select good landmarks: typical choices include random, by high degree, or by high centrality~\cite{sommer2014shortest}.
We next report experiments using the distance-generalized core decomposition as an heuristics to select landmarks. In particular we select  $\ell = 20$ landmarks at random from the core of maximum index (i.e., the $(k,h)$-core such that does not exist a nonempty core $(k',h)$-core with $k' > k$), and we do this for different values of $h \in [1,4]$. We compare with \emph{closeness centrality} ($cc$), which is one of the best-performing heuristics in practice~\cite{Potamias:2009}. For $cc$ we just deterministically select the top-20 vertices.

After having selected  $\ell = 20$ landmarks we measure the approximation error for 500 randomly sampled couples of vertices $s,t \in V$. In particular, we report the relative error that we achieve by approximating $d_G(s,t)$ with the median of the two bounds:
$$
\left( \frac{L(s,t) + U(s,t)}{2} - d_G(s,t) \right) / d_G(s,t).
$$
We also report the so called \emph{triangulation} \cite{kleinberg2004triangulation}, i.e., the ratio $L(s,t) / U(s,t)$ which is a measure of how close the two bounds are: the higher the triangulation, the closer the two bounds, the more accurate is the estimation. As there is stochastic component in the selection of the landmarks, we perform each experiment 10 times and report the average results.

 \begin{table}
 \centering
		\caption{Landmarks selection experiments: approximation error (top-half), triangulation (bottom-half) \label{tab:landmarks}}
	\vspace{-3mm}
	\small
 \begin{tabular}{r|ccccc}
  \multicolumn{1}{c}{} & $h = 1$ & $h = 2$ & $h = 3$ & $h = 4$ & $cc$ \\ \hline %\cline{2-6}
  \texttt{facebook-combined} & 0.25	& 0.16 & 0.12 &	\textbf{0.07} &	0.26 \\
  \texttt{ca-HepPh} & 0.22 & 0.18 & 0.17 & \textbf{0.14} & 0.24 \\
   \texttt{ca-AstroPh} & 0.18 &	0.16 & \textbf{0.14} & \textbf{0.14} & 0.22 \\
   \texttt{douban} & 0.2 &	0.2 & 0.17 & \textbf{0.14} & 0.2 \\
%   \texttt{com-amazon} &  &  &  &  &  \\
%   \texttt{roadNet-PA} &  &  &  &  &  \\
%   \texttt{roadNet-TX} &  &  &  &  &  \\
%    &  &  &  &  &  \\
   \hline
    \texttt{facebook-combined} & 0.25 &	0.3 & 0.35 & 0.39 & \textbf{0.43}\\
  \texttt{ca-HepPh} & 0.27 & 0.34 & 0.35 & \textbf{0.36} & 0.32 \\
   \texttt{ca-AstroPh} & 0.28 & \textbf{0.35} &	0.34 & \textbf{0.35} & \textbf{0.35} \\
   \texttt{douban} & \textbf{0.26} & \textbf{0.26} & 0.25 & 0.25 & \textbf{0.26}\\
%   \texttt{com-amazon} &  &  &  &  &  \\
%   \texttt{roadNet-PA} &  &  &  &  &  \\
%   \texttt{roadNet-TX} &  &  &  &  &  \\
%    &  &  &  &  &  \\
\hline
 \end{tabular}
 \end{table}

Table \ref{tab:landmarks} reports the results over medium-sized datasets for both approximation error (top-half, the smaller the better), triangulation (bottom-half, the higher the better). The results are consistent across experiments, and consistent with the values  of approximation error  and triangulation in the literature. We can observe that in both the metrics, selecting landmarks according to the distance-generalized core decomposition with $h >1$, produces very good landmarks, especially for $h = 4$, which are clearly outperforming the case $h =1$, and are competitive with closeness centrality ($cc$) which is one of the best-performing heuristics reported in the literature.





==> proofs.tex <==
\begin{proof}[Proof of Property \ref{prop:unique}]

By contradiction. Assume there exist two different
$(k,h)$-cores $G[S]=(S,E[S])$ and $G[T]=(S,E[T])$ of $G$.
Consider the subgraph $G[S\cup T]$ induced by the union of $S$ and $T$. It is straightforward that in such subgraph
vertex has at least $k$ neighbors within distance $h$. Thus, also $G[S\cup T]$ is a $(k,h)$-core. It follows that both $G[S]$ and $G[T]$ are not maximal, and thus are not $(k,h)$-cores, contradicting the initial assumption. \end{proof}

\begin{proof}[Proof of Property \ref{prop:subgraph}]

The property follows straightforwardly from the definition of  $(k,h)$-core through the following two observations:
(1) in a subgraph in which every vertex has at least $k+1$
neighbors within distance $h$,  every
vertex also has at least $k$ neighbors within distance $h$ in that subgraph;
(2) as we enlarge the subgraph and add more induced edges, the distance between two vertices may only decrease.
\end{proof} 

\begin{proof}[Proof of Theorem \ref{th:core_club}]

We shall prove by contradiction. Let, if possible, $C$ be an $h$-club of size $k+1$, such that $C=C_1\cup C_2$,
$C_1\cap C_2 = \phi$, and $C \cap \mathcal{C}(k,h)=C_1$. Clearly, $C\setminus \mathcal{C}(k,h)=C_2$.
Let us consider that $\mathcal{C}' =\mathcal{C}(k,h)\cup C_2$.
It is easy to verify that $\mathcal{C}'$ is a $(k,h)$-core of $G$. This is because every node in $C_2$ must
have a path of length at most $h$, to $k$ other nodes of $\mathcal{C}'$, and all these paths will pass through
nodes inside $C \subseteq \mathcal{C}'$. It follows from the definition of $h$-club.
However, this is a contradiction, unless $C_2=\phi$, since our assumption
was that $\mathcal{C}(k,h)$ is the $(k,h)$-core of $G$, and $\mathcal{C}(k,h)\subseteq {\mathcal C}'$. Hence, the theorem.
\end{proof}
